Convergence Analysis and Implicit Regularization of Feedback Alignment for Deep Linear Networks

We theoretically analyze the Feedback Alignment (FA) algorithm, an efficient alternative to backpropagation for training neural networks. We provide convergence guarantees with rates for deep linear networks for both continuous and discrete dynamics. Additionally, we study incremental learning phenomena for shallow linear networks. Interestingly, certain specific initializations imply that negligible components are learned before the principal ones, thus potentially negatively affecting the effectiveness of such a learning algorithm; a phenomenon we classify as implicit anti-regularization. We also provide initialization schemes where the components of the problem are approximately learned by decreasing order of importance, thus providing a form of implicit regularization.

==> app_pics.tex <==



\begin{figure}
    \centering
    \includegraphics[width=.75\textwidth]{./img/theta1theta2_2layer_randTheta0.jpg}
    \caption{Numerical simulation of $50$ solutions of $\theta_2(t)\theta_1(t)$ for FA constant $d=2$, with true label $\lambda=3$ and random initial condition $\theta_0\sim \mathcal{U}([-3,3])$ (the initialization scheme is as in equation \eqref{init_K=0}).}
    \label{fig_randTheta0}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=.75\textwidth]{./img/theta1theta2_2layer_randc2.jpg}
    \caption{Numerical simulation of $50$ solutions of $\theta_2(t)\theta_1(t)$ for random FA constant $d \sim \mathcal{U}([-1,2])$, with true label $\lambda=3$ and initial condition $\theta_0 =1$.
    }
    \label{fig_randc}
\end{figure}





\begin{figure}
    \centering
    \includegraphics[width=.75\textwidth]{./img/2layer_theta0=-2.jpg}
    \caption{Initial conditions $\theta_0 = -2$, FA constants $d =2$. }
    \label{figGissin2l}
\end{figure}




\begin{figure}
    \centering
    \includegraphics[width=.75\textwidth]{./img/2layer_theta0=2.jpg}
    \caption{Initial conditions $\theta_0 = +2$, FA constants $d =2$ }
    \label{figGissin2lbis}
\end{figure}



% \begin{figure}
%     \centering
%     \includegraphics[width=.75\textwidth]{./img/theta0=20.jpg}
%     \caption{Initial conditions $\theta_0 = 20$, FA constants $d =2$ }
%     \label{theta0=20}
% \end{figure}






==> checklist.tex <==
%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{} See Sections \ref{sec3}, \ref{sec4}, \ref{sec5}, \ref{sec6} and supplemental material.
	\item Did you include complete proofs of all theoretical results?
    \answerYes{} See supplemental material: Appendices  \ref{app:FAconv_2layer}, \ref{app:FAconv_Llayers_proof},  \ref{app:impl_reg}, \ref{app:discreteFAconv}.
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{} See Section \ref{sec7}, Appendix \ref{app:experiments} and Google Colab \texttt{.ipynb} file.
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{} See Section \ref{sec7} and Appendix \ref{app:experiments}.
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{} See \figurename\ \ref{fig:autoencoder}.
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{} See Section \ref{sec7}, Appendix \ref{app:experiments} and Google Colab \texttt{.ipynb} file. We worked on the code originally used in \cite{Gidel19}.
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{} See Google Colab \texttt{.ipynb} file.
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{} The original code belongs to one of the authors of the present paper.
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}
